Navigating the Landscape of Hint Generation Research: From the Past to the Future

Digital education has gained popularity in the last decade, especially after the COVID-19 pandemic. With the improving capabilities of large language models to reason and communicate with users, envisioning intelligent tutoring systems (ITSs) that can facilitate self-learning is not very far-fetched. One integral component to fulfill this vision is the ability to give accurate and effective feedback via hints to scaffold the learning process. In this survey article, we present a comprehensive review of prior research on hint generation, aiming to bridge the gap between research in education and cognitive science, and research in AI and Natural Language Processing. Informed by our findings, we propose a formal definition of the hint generation task, and discuss the roadmap of building an effective hint generation system aligned with the formal definition, including open challenges, future directions and ethical considerations.

==> Sections/acknowledgements.tex <==
\section*{Acknowledgements}
ASDF.

==> Sections/recent_developments.tex <==
\section{Survey of Computational Approaches} \label{sec:recent_development}
% \smara{this section should be "Survey of computaitonal approaches" or something like this}
% Despite being a few steps away from creating this ideal education ecosystem, we have made substantial gains with the technological advancements in language technologies.
In this section, we aim to provide a comprehensive overview of the recent developments made by NLP research within the education domain to realize this education ecosystem, with an emphasis on hint generation techniques. We split this section \textbf{into two}, discussing the breakthroughs in the tutoring technologies, and then focus on the developments of selected complementary tasks that might contribute to improvements in the overall tutoring landscape.

% The COVID-19 pandemic, despite its challenges, catalyzed significant advancements in the education sector, emphasizing the value of adaptable curriculum tailored to individual needs, student-focused teaching approaches, and the utilization of both synchronous and asynchronous learning methods \cite{zhao2021changes}. Although we are still a few steps away from creating an ideal education platform that can cater to these needs, we have made some gains with the ever improving language technologies. In this section, we aim to provide a comprehensive overview of the developments made by natural language processing research within the education domain over the last five years, with an emphasis on hint generation techniques. We split this section into two, discussing the breakthroughs in the tutoring technologies, and then focus on the enhancements of selected complementary tasks that might contribute to improvements in the overall tutoring landscape.


% In recent years, the intersection of NLP and education has witnessed remarkable advancements, ushering in a new era of intelligent and personalized learning experiences. As educational technology continues to evolve, NLP plays a pivotal role in enhancing the efficacy of Intelligent Tutoring Systems (ITS) by addressing nuanced challenges in hint generation and adaptive support mechanisms. This section provides a comprehensive overview of the state-of-the-art developments in NLP within the educational domain over the last five years, with a particular emphasis on advancements in hint generation techniques and their integration into AI-based tutoring systems. We split this section into two, discussing the breakthroughs in the tutoring technologies, and then focus on the enhancements of selected complementary tasks that might contribute to improvements in the overall tutoring landscape.

\subsection{Hint Generation Systems}
\smara{this needs to be your main methods section. Create subsections. "Programming", "QA", etc. howeber you want to structure it. and discuss also datasets, methods, and also link to the anatomy of hint, what they actually include and where the gap is.}
A vast majority of explicit hint generation efforts have been focused on the task of programming language domain, owing to the objective nature of the task and abundance of data. Most of the recent efforts in programming hint generation adopt a data-driven deterministic approach \cite{barnes2008toward, rivers2017data, obermuller2021guiding, jin2012program, zimmerman2015automated, paassen2018continuous, price2016generating, rolim2017learning}, that comprises of three key components - a corpus of diverse candidate solutions (usually obtained via past student attempts), a matching algorithm to select the best candidate response given an ongoing attempt based on similarity, and graph-based solution path construction to synthesize hints\footnote{We found abstract syntax tree (ASTs) \cite{mccarthy1964formal, knuth1968semantics} to be the most popular choice of graph-representation for hint synthesis, due to its vast literature and language-agnostic nature.}. 

Two widely popular datasets in the programming hint generation space are \texttt{iSnap} \cite{price2017isnap} and \texttt{ITAP} \cite{rivers2017data} datasets. Both datasets consist of detailed logs collected from several students working on multiple programming tasks, including the complete traces of the code and records of when the hints were requested. \texttt{iSnap} \cite{price2017isnap} is based on the Snap\textit{!} -- a block-based educational graphical programming language, while \texttt{ITAP} \cite{rivers2017data} is a python dataset collected from two introductory programming courses taught at Carnegie Mellon University.

\citet{price2019comparison} develop \texttt{QualityScore}, an evaluation framework that quantifies the quality of programming hints by comparing the generated hints against expert tutor written hints using abstract syntax tree \cite{mccarthy1964formal, knuth1968semantics} based similarity overlap measure. They benchmark the most prominent data-driven techniques on the \texttt{iSnap} \cite{price2017isnap} and \texttt{ITAP} \cite{rivers2017data} datasets, and found the evaluation framework to align well with the expert opinions. \citet{price2019comparison} also identified a few limitations of the benchmarked hint generation systems, such as, a) difficulty identifying the focus of hint request in large code, b) inability to handle divergent code that does not match the existing corpus of past student attempts, and c) inability to understand the student intent. We believe that these are some limitations of using deterministic data-driven techniques, and repurposing latest probabilistic approaches within the neural code synthesis domain such as [cite some code-LLMs] \cite{} might help elevate these shortcomings (refer to Section \ref{sec:future_directions}).

We limit further discussion on programming hint generation systems for brevity, and refer the readers to the surveys written by \citet{mcbroom2021survey}, \citet{crow2018intelligent} and \citet{le2013review} for a comprehensive review.

Beyond programming hint generation, \citet{jatowt2023automatic} proposed a hint generation framework for factoid questions, specifically the “Who?”, “Where?” and “When?” questions. Given a question, the proposed approach extracts the facts about the answer entity from Wikipedia, re-ranks them using popularity-based metrics, and synthesizes hints using pre-determined templates. 
% The proposed approach outperforms randomly selected facts on 30 questions from the SQUAD dataset \cite{rajpurkar2016squad} in a human-evaluation. 
\citet{kochmar2022automated} propose a masking strategy to generate hints, by identifying keywords from the question, and replacing these words in the reference solution by discourse-based template phrases to generate hints. However, this strategy requires reference solutions and their explanations to work effectively. 

Most online education platforms have an ineffective one-size-fits-all framework of education, where everyone is taught the same way \cite{taft2019one}. To overcome this nature of online video learning platforms, \citet{lee2022promptiverse} propose an online learning system called \texttt{Promptiverse}, that provides suitable \textit{scaffolding} hints (referred as `prompts') to give learners a chance to facilitate their understanding about the concept. Promptiverse uses knowledge graphs created on a lecture to create diverse prompts with similar quality to hand-designed prompts, guided by the the learning principles of \textit{Ausubel’s theory on meaningful learning}, that focus on four multi-turn scaffolding principles, namely, \textit{superordinate}, \textit{correlative}, \textit{derivative}, and \textit{combinatorial} prompting \cite{ausubel1963cognitive, 
ausubel1962subsumption, ausubel2012acquisition}.
% \smara{should these be in theory too?}

\smara{again link to hint generation and your desiderata. what was the feedback dimention.}
To quantify the quality of language model's pedagogical capabilities as tutoring dialogue agents, \citet{tack2022ai} proposes a first of its kind evaluation system -- The AI Teacher test. They proposed a human-in-the-loop pairwise comparison test as a solution to this challenging reference-agnostic evaluation task focused on three pedagogical aspects, “\textit{speak like a teacher}”, “\textit{understand a student}”, and “\textit{help a student}”. They identified that the large language models are good at conversation uptake (i.e. the first two requirements), but are quantifiably worse than real teachers on several pedagogical dimensions, especially \textit{helpfulness to a student}.

% The significance of crafting a high-quality dataset becomes evident when considering the development and evaluation of effective hint generation systems in education. A thoughtfully curated dataset should capture a variety of academic subjects and diverse student interactions, offering a nuanced insight into the intricacies of learning patterns. There have been some recent developments to curate high-quality corpus. 
\texttt{ReMath} \cite{wang2023step} is a benchmark developed for evaluating and tutoring students in the mathematics domain. \texttt{ReMath} provides a systematic breakdown of the human-tutoring process into three steps - 1) identifying the type of error, 2) determine a response strategy and intention, and 3) generate a feedback response that adheres to this strategy. \citet{wang2023step} also provide a set of error types (e.g., guess, careless, misinterpret, right-idea etc.), response strategies (e.g., explain a concept, ask a question etc.) and intentions (e.g., motivate the student, get the student to elaborate the answer etc.) to facilitate the feedback generation process. \texttt{ReMath} is a great example of high-quality data collection with human experts towards building better hint generation systems.

% The community currently lacks diverse datasets covering multiple domains. To overcome this scarcity of domain-specific datasets in the education domain, \citet{sakakini2019equipping} proposed Dexter, a tool that extracts subject specific corpus from Wikipedia by relying on a small seed of exemplar instances from the domain of interest.

Even after the substantial progress made in the field of hint generation, there's still a substantial gap between the current technology and real-world applicability of these frameworks. We discuss some other recent endeavours of feedbacks in intelligent tutoring systems and how hint generation can improve these systems in the following section, and the future possibilities of the hint generation landscape in Section \ref{sec:future_directions}.

% Even though hint generation system have made substantial gains over the last couple of years, they still have several limitations that prevent real-world application. Most of the efforts in hint generation are limited to the programming domain, while we are building intelligent tutoring systems beyond that. 

% {\color{blue} TODO - Write passage that mentions the limitations of current hint generation systems, and a segue into why we are exploring feedback in ITSs - mostly to cover their feedback components within the hint generation space, and to draw motivations from them as an auxiliary motive.}

\subsection{Feedback in Intelligent Tutoring Systems} \label{sec:feedback_in_its}
\smara{I mean hints are a type of feedback. You mean otehr type of feedback, is any findings form here relevant to hint generation then say how and related probably to aspects of anatomy of a hint section?}
Feedback in Intelligent Tutoring Systems (ITSs) is crucial for guiding learners' progress and enhancing their understanding through tailored insights and corrective measures. It serves as a dynamic mechanism to provide personalized remarks, helping learners to identify and rectify misconceptions, thus fostering effective learning experiences. 


\citet{grenander2021deep} propose a discourse-aware feedback mechanism, that provides templated responses based on the overlap of elementary discourse units (EDUs) of the student's solution with top candidate solutions. Depending on the excess or deficit of the overlapping EDUs, the system prompts the student to remove or provide additional information respectively. \citet{lee-etal-2023-peep} adopts a two-fold feedback mechanism to provide English learners with feedback on their direct communication abilities. They provide a scalar \textit{context adherence score} measured using semantic similarity of user's response with the current situation, and a \textit{grammatical feedback} modeled as a noise sequence to denoise sequence (NS2DS) framework with copy mechanism \cite{gu2016incorporating}. Similarly, \citet{weber-etal-2023-structured} provides BERT-based \cite{kenton2019bert} classifiers' binary outcomes to develop a writing support system emphasizing on the fundamental elements of appraisal style for the task of writing German legal case solutions. \citet{jin2022stubot} on the other hand develop a learning-by-teaching framework \texttt{StuBot}, where the learners teach the model about a pre-defined topic, and \texttt{StuBot} provides templated feedbacks based on the provided explanations ability to correctly answer some pre-defined questions pertaining to the explained topic. We point the readers to the surveys on ITS for a comprehensive overview of the field.

Although the landscape of intelligent tutoring systems is more diverse than the hint generation literature, most of the recent efforts do not incorporate hints within their feedback mechanism, and merely present the corrected answers, point to the learner's mistakes, or provide a numeric scoring to the responses without explanations. Therefore, we call for further exploration in hint generation to build better intelligent tutoring system that better facilitate the learning needs of learners.

% However, we found that although the landscape of intelligent tutoring systems was more diverse than that of the hint generation, most of the recent efforts do not incorporate hints within their feedback mechanism, and merely present the correct answers or point to the learner's mistakes; overlooking the opportunity to enhance their learning experience. In depth discussion of intelligent tutoring systems is beyond the scope of this paper, and we point the readers to the surveys XYZ in the field for a comprehensive overview.

%  Although these systems could facilitate reasoning in the learning process, these systems have rarely been applied in experimental courses including problem-solving, decision-making in physics, chemistry, and clinical fields. - Source - https://www.tandfonline.com/doi/full/10.1080/10494820.2018.1558257?casa_token=SHmO4tW53ZcAAAAA%3AZmcWgJAe2F2vt-2JKMDAF0xarxjW8Z874vPQn85ioxgBcSQKKbpNKb-Eui6OzJU1NY5F7vYMAHwc

% To overcome the limited opportunities to communicate and practice learnt communication skills for non-native speakers, \citet{lee-etal-2023-peep} designed \texttt{PEEP-Talk}--a real-world situational dialogue-based chatbot to help students learning English as a Foreign Language (EFL) to inculcate direct communication skills. Learners can converse with \texttt{PEEP-Talk} to gain more experience in conversation, and receive feedback--something that non-native speakers might not have enough opportunities to explore otherwise. \texttt{PEEP-Talk} provides a two-fold feedback, a \textit{context adherence score} measured using semantic similarity of user's response with the current situation, and a \textit{grammatical feedback} modeled as a noise sequence to denoise sequence (NS2DS) framework with copy mechanism \cite{gu2016incorporating}. 

% To help foster critical persuasive writing skills within the legal domain, \citet{weber-etal-2023-structured} collected a legal-case using annotator co-developed guidelines, and built several BERT-based \cite{kenton2019bert} classification models to develop a writing support system emphasizing on the fundamental elements of appraisal style for the task of writing German legal case solutions.

% \noindent\textbf{Adopting pedagogical frameworks.}
% \smara{same link to hint generation or desiderata you have for your defintion of hint generation system}
% Studies in the learning sciences have found benefits of \textit{learning-by-teaching} pedagogical mechanism \cite{duran2017learning}. \citet{jin2022stubot} explore this explanatory framework with an LLM-centric approach. They propose \texttt{StuBot}, a conversational agent designed to be taught the learning content by the learners, which then evaluates its tutors by providing adaptive feedback with further questions about the insufficient parts of the explanation text. \texttt{StuBot} is designed to be taught on pre-determined Korean history passages, where feedback is provided based on the model's inability to answer a preset of factoid questions. The model provides feedback if the reading comprehension framework is unable to answer the factoid question based on the provided context. 

% \noindent\textbf{Language acquisition.} 
% \smara{Not clear to me how this whole section is related to hint generation or to elements in your desiderata/formal def you propose for hint generation. You need to link to hint generation}
% Language acquisition is a complex cognitive process and is fundamental to human communication and cultural interaction. With its widespread necessity and deeply rooted theoretical frameworks, language acquisition commands significant attention within the education sector. The advancements in technology is reshaping the way we learn languages, filling in the gaps of traditional education establishments, and augmenting the learner's overall learning experience \cite{golonka2014technologies, chapelle2003english}. Efforts are being made to improve all the major aspects of language education - reading \cite{xiao-etal-2023-evaluating}, speaking \cite{timpe2022using, cardoso2022technology}, listening \cite{hubbard2017technologies, li2023effects} and writing \cite{ryu2020epistolary}. 

% To overcome the limited opportunities to communicate and practice learnt communication skills for non-native speakers, \citet{lee-etal-2023-peep} designed {\color{purple} \texttt{PEEP-Talk}}. A real-world situational dialogue-based chatbot to help students learning English as a Foreign Language (EFL) to inculcate direct communication skills. Learners can converse with \texttt{PEEP-Talk} to gain more experience in conversation, and receive feedback--something that non-native speakers might not have enough opportunities to explore otherwise. \texttt{PEEP-Talk} provides a two-fold feedback, a \textit{context adherence score} measured using semantic similarity of user's response with the current situation, and a \textit{grammatical feedback} modeled as a noise sequence to denoise sequence (NS2DS) framework with copy mechanism \cite{gu2016incorporating}.

% On the other hand, to generate more relatable, personalized, and updated reading material for students to read for language acquisition, \citet{xiao-etal-2023-evaluating} explored the capabilities of LLMs to generate reading comprehension exercises for middle school students. They found the LLM generated text to be suitable for students and comparable to human written text. {\color{purple} [Move to 4.3]}

% Alternatively, \citet{10.1145/1753326.1753567} emphasizes the importance of social supportive behaviors in virtual teaching systems, and develops a robotic tutor that communicates through natural modalities such as speech, gestures and emotional expressions. Their results support the significance of employing \textit{social supportive behavior} in the setting of language learning and acquisition. 

% Language acquisition goes beyond the fundamental ability to speak and write clearly. Professionals in certain domains (like research, law) are expected to cultivate critical writing skills to articulate persuasive arguments, analyze complex legal issues, and effectively communicate their insights. To help foster these critical persuasive writing skills, \citet{weber-etal-2023-structured} collected a legal-case using annotator co-developed guidelines, and built several BERT-based \cite{kenton2019bert} classification models to develop a writing support system emphasizing on the fundamental elements of appraisal style for the task of writing German legal case solutions. [This can be classified as hints/indicators to aid the writing process.]

% However, \citet{weber-etal-2023-structured} raises the concerns of low supervision ratio in the legal education system, and develops a structured persuasive writing support tool based on a dataset of legal case solutions collected at a German law institution.

% \noindent\textbf{Adopting pedagogical frameworks.}
% \smara{same link to hint generation or desiderata you have for your defintion of hint generation system}
% Studies in the learning sciences have found benefits of \textit{learning-by-teaching} pedagogical mechanism \cite{duran2017learning}. \citet{jin2022stubot} explore this explanatory framework with an LLM-centric approach. They propose \texttt{StuBot}, a conversational agent designed to be taught the learning content by the learners, which then evaluates its tutors by providing adaptive feedback with further questions about the insufficient parts of the explanation text. \texttt{StuBot} is designed to be taught on pre-determined Korean history passages, where feedback is provided based on the model's inability to answer a preset of factoid questions. The model provides feedback if the reading comprehension framework is unable to answer the factoid question based on the provided context. 
% \texttt{StuBot}, although a domain-agnostic system, was evaluated on the topic of middle-school-level Korean history due to the participants' familiarity.

% Another popular dataset is \texttt{CoAuthor} \cite{lee2022coauthor}, a large scale \textit{model interaction dataset} developed between 63 writers and GPT-3 for the tasks of creative writing and argumentative writing. The interactive nature of the datasets helps unveil insights on the collaborative capabilities of LLMs in writing assistance varying from improving the vocabulary diversity to enhancing the ideation capabilities. The authors also collect the writer's perception as a part of their data pipeline, which unveils findings otherwise impossible. \textit{E.g.,} the writer’s perceived using GPT-3 to increase their productivity, and they found that adopting GPT-3’s suggested edits lead to a lower perceived ownership. 
% \smara{Is coAuthor about hints? Or is it in general writing assistance (it is not knowledge testing it is a different task) so again you might want to have hint generation for different "learning objective"- concept learning, writing skills acquisition, language acquisioton. etc}

% Although \texttt{ReMath} and \texttt{CoAuthor} are useful in their respective tasks, however, the community currently lacks diverse datasets covering multiple domains. To overcome this scarcity of domain-specific datasets in the education domain, \citet{sakakini2019equipping} proposed Dexter, a tool that extracts subject specific corpus from Wikipedia by relying on a small seed of exemplar instances from the domain of interest.
% \smara{how is this relevant to hint generation, everything you mention you need to link to your task and the formal definition you propose}

% \textbf{Student feedback analysis.}
% Student feedback is essential to the educators, as it helps them modify their teaching style and reform their course structure. 
% Beyond developing effective tutoring systems, datasets and their analysis, it is also important to help give student's feedback to the educators, helping them modify their teaching style and reform their course structure by accounting for students’ feedback. 
% However, in online education platforms, student feedback is often present in an unstructured manner, making it difficult to gain useful insights. To overcome this, \citet{wang-etal-2023-sight} proposed to use LLMs to sift through the unstructured student feedback (comments on the education platforms), and finds LLMs to be highly correlated with human annotators on a predefined qualitative assessment rubric. They also release the \texttt{SIGHT} (Student Insights Gathered from Higher Education Transcripts) dataset, with the transcribed MIT OpenCourseWare lectures, user comments, and LLM’s qualitative codes.
% \smara{again how is this linked to any aspects of your proposed defintion}

% \noindent\textbf{Beyond schools.} However, the impact of education goes beyond teaching establishments like schools; humans are constantly learning, acquiring new knowledge for continuous improvement \cite{ahmed1999cultures}. For instance, \citet{gupta-etal-2020-heart} collect data and perform qualitative analysis of experts towards educating African American and Hispanic/Latino patients coping with heart failures in a culturally sensitive and linguistically accurate manner. 

\subsection{Advancements in Complementary Tasks}
\smara{I won't have such a section, Rather you will have a Roadmap to future research in hint generation where you have desiderata (e.g. reasomning an mention current reasoning advances and where next; multimodality, where we are and what is next etc}
In this section, we aim to briefly describe selected complementary efforts within the NLP community that can improve the quality of hint generation systems today (refer to Fig. \ref{fig:overview}).
% In the dynamic landscape of education technology, integration of NLP techniques have expanded the horizons of new possibilities, revolutionizing the ways learners engage with educational content. This section delves deeper into the advent of some influential directions within the NLP community that might support the development of successful hint generation systems and effectively the intelligent tutoring systems.

\noindent\textbf{Answer Assessment}\newline
Answer assessment plays a pivotal role in evaluating and understanding learner responses, enabling the system to provide targeted feedback and adaptive guidance. Accurate answer assessment is foundational for standardizing the grading process, identifying misconceptions, tracking individual progress, and tailoring subsequent hints to address specific learning needs. Evaluating a learner's responses is by no means an easy task; depending on the length and technical complexity of the system, the approach to evaluate answers can vary drastically. 
Although there exist plenty of efforts in answer matching for question answering systems and evaluation of text summarization systems for longer text forms, very few have been applied in the context of student answer assessment. For short form text, \citet{bulian2022tomayto} illustrate that the most commonly adopted answer assessment techniques like Exact Match and Token F1 are not ideal, and adopt a semantic BERT-based [CITE] approach to illustrate the asymmetric notion of the task. On the other hand, \citet{li2023distilling} successfully distilled the reasoning abilities of LLMs [CITE ChatGPT] in generating rationales, and trained smaller T5 models [CITE] to develop explainable answer assessment models. To reduce the marking workload of teachers, \citet{chang2022towards} proposed a semantic grouping of multiple learners’ responses for batch grading to reduce the evaluation workload from teachers; limiting the study to short answers consisting of 1-2 sentences. Beyond text-centric education, with the advent of online education in a post-COVID era [\textbf{cite relevant paper}], oral presentations have also become an integral part of the virtual education system \cite{liu2020recent}. To provide a personalized feedback across several modalities of an oral presentation (namely text, images/slides, audio), \citet{liu2020personalized} propose a multi-modal feedback generation system to provide more fine-grained assessment to student submissions. These approaches, albeit valuable to the community, still lack the performance and reliability required to be deployed in the real-world ITS systems.

\noindent\textbf{User Modeling} User modeling is quite extensively explored within the realm of recommendation systems, with the aim to adapt and customize a service to user's specific needs. User modeling holds the key to identifying the learner's interests and preferences within the hint generation space. \citet{liu2022open}, for instance, utilizes long short-term memory (LSTM) cells [CITE] to for knowledge estimation \cite{corbett1994knowledge} of student's current understanding based on their past responses for open-ended program synthesis. We believe that using similar strategies to model student's progress would help enhance their learning experience, and direct the readers to comprehensive surveys authored by \citet{li2021survey} and \citet{he2023survey} for an extensive overview.

\noindent\textbf{Dialogue systems} Intelligent tutoring systems are mediated by dialogue systems (or conversational agents), providing an interface between ITS and learners. With the recent developments in retrieval augmented generation [CITE], emotion-aware dialogue systems [CITE], enhanced language understanding capabilities [CITE] and long-term dependencies, dialogue systems today can also help improve the hint generation systems, empowering them with abilities to better understand the learner's queries, understand and respond to complex domains, generate affective responses, and keep track of long conversation sessions for adaptive tutoring. For further exploration, we guide the readers to the surveys written by \citet{ni2023recent}, \citet{deriu2021survey} and \citet{ma2020survey}.

\noindent\textbf{Question generation.} Questions play pivotal roles in education, serving to recall knowledge, test comprehension, and foster critical thinking. \citet{AlFaraby2023} classify neural question generation for educational purposes into three broad categories - Question Generation from Reading Materials, Word Problem Generation, and Conversation Question Generation. We posit a similar use case for question generation to generate hints within conversations, to clarify not just the learner's response, but also their understanding and ability to present their ideas. We point the readers to surveys written by \citet{kurdi2020systematic}, \citet{zhang2021review}, \citet{das2021automatic} and \citet{pan2019recent} for a comprehensive overview.

\noindent\textbf{Reasoning in LLMs.} Large language models (LLMs) have exhibited the abilities to reason when they are sufficiently large, enabling them to perform various forms of reasoning, including logical reasoning, inference, and problem-solving. Their ability to reason helps them analyze complex textual data, extract relevant information, and generate coherent responses, making them a valuable tool for educational applications such as hint generation. With the help of this reasoning abilities, we are now closer to equipping hint generation systems with the ability to provide personalized remarks, generate contextually relevant hints, and engage in interactive conversations with the learners. To gain a comprehensive understanding, readers are encouraged to explore surveys on reasoning in LLMs \cite{huang2022towards,zhang2023igniting}.

\noindent\textbf{Student Feedback Analysis.} Student feedback is essential to the educators, as it helps them modify their teaching style and reform their course structure. 
% Beyond developing effective tutoring systems, datasets and their analysis, it is also important to help give student's feedback to the educators, helping them modify their teaching style and reform their course structure by accounting for students’ feedback. 
However, in online education platforms, student feedback is often present in an unstructured manner, making it difficult to gain useful insights. To overcome this, \citet{wang-etal-2023-sight} proposed to use LLMs to sift through the unstructured student feedback (comments on the education platforms), and finds LLMs to be highly correlated with human annotators on a predefined qualitative assessment rubric. They also release the \texttt{SIGHT} (Student Insights Gathered from Higher Education Transcripts) dataset, with the transcribed MIT OpenCourseWare lectures, user comments, and LLM’s qualitative codes.

% \smara{do you need also advances in user-modeling, dialog generation, question generation, reasoning, etc?}

==> Sections_v1/introduction.tex <==
\section{Introduction} \label{sec:intro}

% Para 1 - What are hints, and their role in tutoring/education.
% Para 2 - Motivate ITS - bad ratio, expensive personalized tutoring.
% Para 3 - How NLP can play a role in developing better hint generation systems. How education has been affected by NLP. Hint are critical part of conversation. 
% Para 4 - survey overview and major contributions.
\smara{Main points: Intro needs a bit more clarity what what are hints and why they are important in education/learning. Then say this paper focuses on a review of current computational approaches for hint generation models/datasets/domains/hint types, and a    roadmap for the future including a rethinking of a formal defintion of hint generation process. Then we the have section 2 Anatomy of the hint, where after each paragrapah we say the hint generation will need x, y “user background knowledge” or “history of hints”  (and you can mention notation too which you then later connect to formal definition). Then Section 3 it is Survey on computational models particularly foused on hint generation: 3.1 Hint Generation: this has to be the biggest part with clear subsection: 3.1.1 Programming Hint and more details and point back of how the incorporate elements from anatomy of a hint. Btw, the survey there were also describing type of hints: correcting errors, etc (we should do that too).  Also datasets 3.1.2 Open-domain Hints (QA) : I assume here is only correcting errors. Here mention they have a formal definition and what they do. 3.1.3 visual prompts etc, whatever you have left. This section needs to discuss domain, hint types, models, datasets etc. Then in 3.2 Other feedback mechanism beside hints ? (why  you want to mention them?  and link to elements to Anatomy of  hint).  You should remove  complementary tasks from Section 3, you will mention some of them when needed in your Section 4. “Roadmap for future research in Hint generation” . There you have 4.1 Rethinking formal definition ; and then 4.2. A Hint Generation system (and all those features you have an there you mention relevant research (e.g. in reasoning, multimodality etc). Herei s a nice survey in a different domain that had a conceptialization component. they map the literatue into the conceptualization to show gaps/status etc. https://aclanthology.org/2022.in2writing-1.2.pdf }

Prior research has established a correlation between the student-teacher ratio and student's overall performance \cite{koc2015impact}. However, private tutoring is not accessible to everyone, and finding expert tutors is often difficult. 
%infeasible in many cities. 
Intelligent tutoring systems (ITSs) have the capabilities to address these educational challenges, notably the need for personalized learning in a system often reliant on didactic teaching and standardized testing. Modern ITSs are adaptive instructional systems that leverage artificial intelligence techniques together with pedagogical strategies to provide a personalized tutoring experience to trigger a cognitive and motivational change in the student.
\smara{you need citations to all the above sentences}

The hallmark of intelligent tutoring systems is their ability to provide next-step help to students while they work on problems, and hints play a critical role in their ability to provide this help. \smara{add citations here; also is next-step or "step-by-step"} Hints in education refer to the clues, prompts, questions, or suggestions provided to learners to aid them in solving problems, answering questions, or completing tasks, thereby encouraging critical thinking, problem-solving skills, and independent learning \smara{add citations}.They are a tool to provide scaffolded support to the learners, and can be traced back to the socio-cultural theory of Vygotsky’s Zone of Proximal Development (ZPD), referring to "the gap between what a learner can do without assistance and what a learner can do with adult guidance or in collaboration with more capable peers" \cite{lev1979mind}. This framework of scaffolding is well-established within the education space \cite{van2010scaffolding}, and expert tutors are often guided to incorporate it in their teaching practices \cite{belland2017instructional}.

% Recent technological advances and adoption of e-learning platforms post COVID-19 emergency have increased popularity of research to build intelligent tutoring systems (ITSs). The goal of these intelligent tutoring systems is to replicate the demonstrated benefits of one-to-one personalized tutoring to provide high quality education in an accessible manner. An integral part of this one-to-one tutoring is the expert tutor's ability to give personalize feedback to the learners to help develop higher cognitive skills and problem-solving abilities efficiently. Hints are often utilized as a scaffolded supports to provide this feedback, designed to offer just enough guidance to help learners progress without providing the complete solution.

Natural Language Processing (NLP) has made significant impact on the education landscape and intelligent tutoring systems, with developing human-like conversational agents that help facilitate conversation with users to large-scale retrieval frameworks that empower these dialogue agents with vast world knowledge. However, there are some fundamental gaps in the NLP-empowered ITSs, and in this interpretive survey, we aim to discover these shortcomings and provide future directions to foster better intelligent tutoring systems grounded in the pedagogical approaches and cognitive theories of human learning. \smara{is interpretive survey a term? are we proposing ITS? should we just frame around hint generation as a form of feedback mechanism in ITS}
\smara{shpould we just say here we will provide a survey on hint generation looking at problem domains (programming vs. QA vs. concept learning vs. etc), methods, datasets. We identify gaps and propose a roadmap  for future research hint generation including a rethinking of formal defintion of hint generation introduce in \cite{}. Something like this }
In contrast to prior surveys on programming hint generation \cite{mcbroom2021survey, crow2018intelligent, le2013review}, we aim to explore the possibilities of hint generation beyond the deterministic solution space of programming languages, exploring the possibilities of hint generation in other subjects such as natural sciences, social sciences, language acquisition etc. -- the domains seldom explored in the ITS literature \cite{mousavinasab2021intelligent}. In this timely literature review, we aim to cover the recent efforts in hint generation and relevant neighboring fields to provide a comprehensive understanding of the field for interested scholars to gain insights and shape future efforts in this field. \smara{remove "timely" you can rework this once the overall structure change}

Our paper makes three main contributions: 
\begin{enumerate}
    \item We survey recent papers on automatic hint generation and complementary tasks to provide a comprehensive understanding of the field. 
    \item We provide a formal definition for the hint generation task, grounded in cognitive theories on learning and qualitative research within the education and learning sciences.
    \item We accentuate open challenges in current hint generation systems and outline promising future directions for this field.
\end{enumerate}

% Acknowledge the vast research in dialogue technology, and tutoring systems; but state the significance of studying hint generation separately as the atomic unit of feedback that targets the cognitive development.

% \textbf{Todo item} - Create a figure to explain hint generation, and its complexity. Use examples to do so.


% Paragraph 1 - Motivate the hint generation problem within the education space from cognitive sciences aspect of learning and knowledge acquisition. Also describe the problem of hint generation in layman's terms. Use ACT-R theory to motivate the importance of feedback beyond providing the correct answers.

% Paragraph 2 - Mention the advances in NLP, shortcomings of education sector in some aspects, and how we can adopt recent advances to develop better hint generation systems. Address the other surveys on programming language, but how they have a limited scope, and there's value in this "timely" survey.

% Paragraph 3 - Importance of doing this research, overview of the survey, and major contributions.

% The notion of intelligent tutoring systems has been studied for over half a century, 

% In this survey, we aim to study the nuances of automatic hint generation process, and provide a comprehensive review of the field.

% Hints are a very prominent and essential component of these intelligent tutoring systems, aiming to provide guidance and feedback to reduce the task complexity delicately to match the learner's cognitive abilities. 

% We describe an example of a hint generation system for natural answers in Figure \ref{fig:intro-fig}, where it acknowledges a learner's response, and guides them into correct information by mentioning "insulin" to bridge the association of diabetes and pancreas. 

% to replicate the demonstrated benefits of one-to-one personalized tutoring to provide high quality education in an accessible manner. 

% Internet-based education has gained a lot of traction in the last decade, due to the advances in technology and the COVID-19 emergency [CITE]. This increased popularity of e-learning technologies have also motivated research to build better intelligent tutoring systems (ITSs), that aims to replicate the demonstrated benefits of one-to-one personalized tutoring to provide high quality education in an accessible manner. Feedback is a vital component of these intelligent tutoring systems \cite{dabolicnvs2013role}, with the aim to provide personalized remarks to improve the learner's understanding. One prominent form of providing feedback for guidance is hints, aiming to reduce the complexity of the task delicately to match the learner's cognitive abilities. Hints are a consequence of scaffolding in education, which can be traced back to the Vygotsky’s Zone of Proximal Development (ZPD), described as “\textit{the distance between the actual developmental level as determined by independent problem solving and the level of potential development as determined through problem solving under adult guidance or in collaboration with more capable peers}” [CITE].

% In this timely survey, we cover the recent computational advancements in hint generation systems, while 

% be it large-scale analysis of student feedbacks, answer assessment systems, or aiding language acquisition through machine translation. In this paper, we focus on specific advancements in NLP that can help build better hint generation systems, such as 

% The field of natural language processing has made great advancements over the last decade with the advent of large language models (LLMs) such as ChatGPT, Geminai, Mistral, OLMo, etc. achieving state-of-the-art performance on several benchmarks. We believe that making use of these LLMs and other advances in neural computational science, we can improve the existing hint generation systems and expand this line of research beyond what's been explored so far. 

% In this survey we aim to bring together the efforts in the learning and education sciences, and the NLP community to foster better research to enhance the online intelligent tutoring systems. We survey the ongoing research in hint generation and neighboring fields that we feel are relevant to the future of the task, and present a 

% In contrast to existing surveys [CITE], this paper expands on hint generation beyond programming domain, exploring the possibilities of hint generation system in other education domains such as language acquisition, science, social science, mathematics etc. while being grounded to the learning and cognitive sciences.

Random lines for introduction - 
\begin{enumerate}
    \item An ideal education ecosystem should emphasize on the value of adaptable curriculum tailored to individual needs, student-focused teaching approaches, and the utilization of both synchronous and asynchronous learning methods \cite{zhao2021changes}. 
\end{enumerate}
